Scenic Routes over Points in 2D Space

Consider a 2D coordinate space with a set of red and a set of blue points. We define a scenic point as a point that is equidistant to a red point and a blue point. The set of contiguous scenic points form a scenic path. The perpendicular bisectors to the line joining a red point and a blue point forms a scenic path between the red point and the blue point. A scenic route is a traversal made from scenic paths. In this paper, we address this novel problem by (i) designing algorithms for scenic route generation, (ii) studying the algorithms different properties and (iii) analyzing the routes generated by these algorithms. Scenic routes have applications in geo-spatial visualizations and visual analytics.

==> text/problem.tex <==
\section{Problem Scope}
\label{sec:problem}
\vspace{5pt}
\subsection{\textbf{Problem Introduction}}
\label{ssec:problem_intro}
Consider a rectangular region with $N$ red and $M$ blue points. We define a  \bo{scenic point} as a point that is equidistant to at least one pair of red-blue points. A path on which each point is scenic is termed as a \bo{scenic path}. Likewise, a collection of scenic paths forms a \bo{scenic route}. Each point on the perpendicular bisector of a line joining a pair of red-blue points is scenic. Therefore, the entire perpendicular bisector is a scenic path. Scenic routes are generated by putting together segments of these bisectors/scenic-paths. The intersection points of multiple bisectors offer multiple scenic views as they produce an equidistant view to multiple pairs of points. Moreover, these intersection points offer opportunities to change directions, i.e., move from one bisector to another while maintaining a scenic view.

In this paper, we propose methods to find scenic routes in 2-dimensional regions. Since the routes must be scenic, we can ignore the actual red-blue points and only focus on the bisectors and the points where the bisectors intersect. Moreover, we can transform this set of intersection points into a graph connected by the bisectors forming a "scenic graph". A traversal over such a scenic graph would give us a scenic route.

\begin{figure}[!t]
    \center
    \includegraphics[width=\linewidth]{images/start_example.png}
    \caption{}
    \label{fig:start}
\end{figure}

% We delve into multiple possibilities, such as routes that minimize total travel distance, routes that include long, straight paths, among others. We present several algorithms to generate these routes.

\subsection{\textbf{Mathematical Framework}}
\label{ssec:problem_math}
Let the set of red points be $R$, the set of blue points be $B$ and the set of points where the bisectors intersect be $I_P$. Segments of the bisectors between these intersection points form the edge set $E_P$ which contribute as edges of the scenic paths. The weight of each edge is the Cartesian distance between its endpoints. 

%Old statement: The set of edges (scenic paths) between these intersection points(which are segments of the bisectors) is represented using $E_P$ where the weight of each edge is the Cartesian distance between its endpoints. 

% RESOLVED, REPLY BELOW Loay: Here edges are segments of a bisector but it can become a segment only if the line is bound on both sides so is bounding box marking one end of the bisectors?
% \llini{"Is bounding box marking one end of the bisectors?" Theoretically yes. But in my implementation, no. The bounding box restricts the $I_P$ and the edges in $E$ are drawn from the remaining intersection points. It is as if the intersection points outside the bounding box never existed.}

The graph over all the intersection points is $G(I_P, E_P)$. Moreover, for a selected route; let the set of points on a route be $S \subset I_P$, and the edges within the route be $E \subset E_P$. We represent a scenic route as a graph using the notation: $G(S, E)$.
% SEEN Loay: made it $E \subset E_P$.

We explain the problem further by using Figure \ref{fig:start}. Consider the point configuration containing 1 red point $\{R_1\}$ and 3 blue points $\{B_1, B_2, B_3\}$. $\{M_1, M_2, M_3\}$ represent the midpoints of the lines joining them. The green lines are the perpendicular bisectors of these lines. The green lines represent scenic paths. The intersection points of these perpendicular bisectors have been represented using $\{IP_1, IP_2, IP_3\}$. Therefore, to obtain a scenic route, we consider the perpendicular bisector, and to move from one bisector to another, we use their intersection points. In this case:
% \begin{align*}
% I_P &= \{IP_1, IP_2, IP_3\} \\
% E_P &= \{[IP_1 IP_2],\ [IP_2 IP_3],\ [IP_3 IP_1]\}
% \end{align*}
$$I_P = \{IP_1, IP_2, IP_3\}$$
$$E_P = \{[IP_1 IP_2],\ [IP_2 IP_3],\ [IP_3 IP_1]\}$$

The corresponding graph is $G(I_P, E_P)$. Edges and points within a scenic route are in pink.

\subsection{\textbf{Paper Contribution and Layout}}
\label{ssec:problem_contrib}
The contribution of this paper are (1) the introduction of scenic routes (based on the equidistant principle) in two-class point configurations in 2D spaces (2) various scenic route generation algorithms fulfilling different requirements. 
% The points of interest can be changed from two-class to multi-class and the algorithms will still hold true, without loss of generality.

In Section \ref{sec:routes} we delve into the meaning of scenic routes and lay down requirements for a route to be considered as scenic. Section \ref{sec:algorithms} contains objectives, explanations, and the motivations behind each algorithm. Section \ref{sec:dicussion} then discusses how well the routes generated using our algorithms perform on the scenic requirements. Section \ref{sec:spatial} deals with possible spatial restrictions that can be applied to $I_P$. The Appendix contains pseudocodes for all the presented algorithms.
%UNABLE TO LINK APPENDIX

==> text/questions.tex <==
\section{Open Questions}
\label{sec:questions}

We present a number of open questions regarding the work here.
